Desingularization of the Milne Universe

Resolution of cosmological singularities is an important problem in any full theory of quantum gravity. The Milne orbifold is a cosmology with a big-bang/big-crunch singularity, but being a quotient of flat space it holds potential for resolution in string theory. It is known however, that some perturbative string amplitudes diverge in the Milne geometry. Here we show that flat space higher spin theories can effect a simple resolution of the Milne singularity when one embeds the latter in 2+1 dimensions. We explain how to reconcile this with the expectation that non-perturbative string effects are required for resolving Milne. Along the way, we introduce a Grassmann realization of the \.{I}n\"on\"u-Wigner contraction to export much of the AdS technology to our flat space computation.

==> acknowledgement.tex <==
CK thanks Arjun Bagchi, Ben Craps, Justin David, Oleg Evnin, Jarah Evslin, Prem Kumar and Boris Pioline for discussions, and Chalmers Institute of Technology, Sweden and the Yerevan State Univeristy, Armenia (during the ``Quantum Aspects of Black Holes and its Recent Progress" worskhop) for hospitaility during parts of this work. The research of SR is supported by Department of Science and Technology (DST), Govt.$\hspace{0.05in}$of India research grant under scheme DSTO/1100 (ACAQFT).

